On the Interplay between Social Welfare and Tractability of Equilibria

Computational tractability and social welfare (aka. efficiency) of equilibria are two fundamental but in general orthogonal considerations in algorithmic game theory. Nevertheless, we show that when (approximate) full efficiency can be guaranteed via a smoothness argument \`a la Roughgarden, Nash equilibria are approachable under a family of no-regret learning algorithms, thereby enabling fast and decentralized computation. We leverage this connection to obtain new convergence results in large games -- wherein the number of players $n \gg 1$ -- under the well-documented property of full efficiency via smoothness in the limit. Surprisingly, our framework unifies equilibrium computation in disparate classes of problems including games with vanishing strategic sensitivity and two-player zero-sum games, illuminating en route an immediate but overlooked equivalence between smoothness and a well-studied condition in the optimization literature known as the Minty property. Finally, we establish that a family of no-regret dynamics attains a welfare bound that improves over the smoothness framework while at the same time guaranteeing convergence to the set of coarse correlated equilibria. We show this by employing the clairvoyant mirror descent algortihm recently introduced by Piliouras et al.

==> text/applications.tex <==
\section{Applications}

In this section, we present several applications of our main result based on some earlier results that quantify the efficiency of Nash equilibria in large games~\citep{Feldman16:The,Cole16:Large}.

\subsection{Simultaneous uniform-price auctions}
\label{sec:uniform-price}

First, based on the work of~\citet{Feldman16:The}, we consider a market with $n \in \N$ bidders and a number of $m \in \N$ different types of goods (or items). For each good $j \in \range{m}$ there are $k_j^n \in \N$ units of that good. Each player $i \in \range{n}$ is associated with a valuation function $v_i : \N^{m} \to [0, V]$, for some parameter $V > 0$, which assigns a value to each different bundle of goods, depending on the number of units of each good. In particular, it is assumed that players have bounded demand for each good, so that if $\vx_i \in \N^m$ is the allocation vector of bidder $i$, it holds that $v_i(\vx_i) \equiv (\min\{\vx_i(1), r\}, \dots, \min \{ \vx_i(m), r\} )$, for some (commonly known) parameter $r \in \N$. For convenience, it is also assumed that the valuations are bounded away from $0$ for any nonzero allocation vector $\vx_i \neq \vec{0}$, in that $v_i(\vx_i) \geq \rho > 0$.

In this context, a mechanism $\cM$ consists of the triple $( (S_i)_{i=1}^n, (\vx_i)_{i=1}^n , (P_i)_{i=1}^n)$, where $S_i$ is the strategy space of player $i \in \range{n}$ and $S \defeq \prod_{i=1}^n S_i$; $\vx_i$ is the allocation function corresponding to player $i$, which maps a joint strategy profile $\vec{s} \in S$ to a feasible allocation; and $P_i : S \to \R_{\geq 0}$ is the payment function. The utility of a bidder\io{decide between bidder and player} is defined as $u_i(\vec{s}, v_i) \defeq v_i(x_i(\vec{s})) - P_i(\vec{s})$, while the social welfare is the total value received by the bidders under mechanism $\cM$: $\sw(\vec{s}, v) \defeq \sum_{i=1}^n v_i(x_i(\vec{s}))$. Finally, the revenue of a mechanism is defined as the sum of the payments, that is, $\cR(\vec{s}) \defeq \sum_{i=1}^n P_i(\vec{s})$. \io{definition of Bayes-Nash} 

\begin{definition}[Smoothness for mechanisms~\citep{Syrgkanis13:Composable}]
A mechanism $\cM$ is $(\lambda, \mu)$ smooth if for any valuation profile $\vec{v} \in \prod_{i=1}^n \cV_i$ there is a joint strategy $\vsstar \in S$ such that for any strategy $\vs \in S$,
\begin{equation*}
    \sum_{i=1}^n u_i(\vsstar_i, \vs_{-i}; v_i) \geq \lambda \opt(\vec{v}) - \mu \sum_{i=1}^n P_i(\vs).
\end{equation*}
\end{definition}

Moreover, all Bayes-Nash equilibria in a $(\lambda, \mu)$-smooth mechanism attain at least a $ \rpoa_{\cM} \defeq \frac{\lambda}{\max\{1, \mu\}}$\io{You should take the infimum here} fraction of the optimal social welfare~\citep{Syrgkanis13:Composable}.

We return to the description of simultaneous\io{Important to check if this applies for sequential auctions as well} uniform-price auctions. The units of each good $j \in \range{m}$ are disposed simultaneously and independently through a uniform-price auction. More precisely, the auctioneer elicits $r$ bids $\vb_{i, j}(1) \geq \dots \geq \vb_{i, j}(r)$ from each bidder $i$, referred to as the marginal bids. Then, each bid that was amongst the $k_j^n$ highest ones receives a unit; \io{ties are broken randomly}. Every bidder is charged the highest losing bid of an item for every unit allocated to that bidder. We will assume that every bid is at most a fixed number $B$; we note that it is a weakly dominated strategy to not bid above $V$. The bidding set of each player will be denoted by $\cB$.\io{$\cB$ has small diameter and allows efficient projections} This auction format is clearly not truthful, as it does not even allow the bidders to express their real valuations.

\subsection{Walrasian auction}

For an allocation $\vx_i$ to bidder $i$, we write $\vx_i(j) \in \N \cup \{0\}$ to denote the number of copies of good $j \in \range{m}$ received by $i$ under allocation $\vx_i$. A mechanism $\cM$ computes a vector of prices $\vec{p} = (p_1, \dots, p_m)$, one for each good. Every bidder has a valuation function $v_i : X \to \R_{\geq 0}$, where $X$ is the set of all possible allocations. Bidders are further assumed to have quasilinear utility functions $u_i(\vx_i; v_i) \defeq v_i(\vx_i) - \langle \vx_i, \vec{p} \rangle$.

\begin{definition}[Walrasian equilibrium]
    A vector of prices $\vec{p} = (p_1, \dots, p_m)$ and an allocation $\vx = (\vx_1, \dots, \vx_n) \in X$ is a Walrasian equilibrium if 
    \begin{itemize}
        \item the goods are fully allocated but not over-allocated: $\sum_{i=1}^n \vx_i(j) \leq k_j$ for all $j \in \range{m}$, with equality only when $p_j > 0$; and every bidder $i$ is maximize its own utility at the current price $\Vec{p}$:
        \item $u_i(\vx_i; v_i) = \max_{\vx_i'} \{ v_i(\vx'_i) - \langle \vx_i', \Vec{p} \rangle \}$.
    \end{itemize}
\end{definition}

\begin{definition}[Gross substitutes]
    A valuation or a bid function satisfies the gross substitutes property if increasing the price of one good can only increase the demand for the other goods.
\end{definition}

The key property that characterizes a large Walrasian auction---in the sense of~\citet{Cole16:Large}---is \emph{anti-concentration}: the number of copies $k_j$ of each item $j \in \range{n}$ follows a distribution $F$ such that $\pr_F[k_j = \kappa] \leq \frac{1}{L}$, for any $\kappa \in \N \cup \{0\}$, for some parameter $L$. In particular, $L$ measures the ``largness'' of the underlying auction, analogously to the role of the number of bidders we encountered earlier in~\Cref{sec:uniform-price}.

\begin{assumption}[Bounded expected value]
    \label{ass:bounded_value}
There is a parameter $V \in \R_{> 0}$ such that for each bidder $i$ and item $j \in \range{m}$,
\begin{equation*}
    \E_{v_i \sim \cV_i} [v_i(j)] \leq V.
\end{equation*}
\end{assumption}
